Streaming Submodular Maximization under Matroid Constraints

Recent progress in (semi-)streaming algorithms for monotone submodular function maximization has led to tight results for a simple cardinality constraint. However, current techniques fail to give a similar understanding for natural generalizations, including matroid constraints. This paper aims at closing this gap. For a single matroid of rank $k$ (i.e., any solution has cardinality at most $k$), our main results are: 1) a single-pass streaming algorithm that uses $\widetilde{O}(k)$ memory and achieves an approximation guarantee of $0.3178$, and 2) a multi-pass streaming algorithm that uses $\widetilde{O}(k)$ memory and achieves an approximation guarantee of $(1-1/e - \varepsilon)$ by taking a constant (depending on $\varepsilon$) number of passes over the stream. This improves on the previously best approximation guarantees of $1/4$ and $1/2$ for single-pass and multi-pass streaming algorithms, respectively. In fact, our multi-pass streaming algorithm is tight in that any algorithm with a better guarantee than $1/2$ must make several passes through the stream and any algorithm that beats our guarantee of $1-1/e$ must make linearly many passes (as well as an exponential number of value oracle queries). Moreover, we show how the approach we use for multi-pass streaming can be further strengthened if the elements of the stream arrive in uniformly random order, implying an improved result for $p$-matchoid constraints.

==> tex/twoPlayerMatStreaming.tex <==
\section{Better-than-\texorpdfstring{$2$}{2} approximation for two-player submodular maximization subject to a matroid constraint} \label{sec:twoplayer}

Let $M=(\cN,\mathcal{I})$ be a matroid with rank function $r\colon 2^\cN \to \mathbb{Z}_{\geq 0}$, let $k\coloneqq r(\cN)$ be the cardinality of a basis of $M$, and let $f\colon 2^\cN \to \mathbb{R}_{\geq 0}$ be a non-negative submodular function. We are interested in maximizing $f$ under the matroid constraint $M$ in the following two-player setting. The ground set $\cN$ is partitioned into two sets $\cN=\cN_A \cup \cN_B$. The first player, Alice, obtains $\cN_A$ and can query $f$ on any subset of $\cN_A$. She then selects a subset of elements $Q\subseteq \cN_A$ to be forwarded to the second player, Bob. After receiving the elements forwarded by Alice, Bob returns an independent set $R\in \mathcal{I}$ with $R\subseteq Q\cup \cN_B$. The goal of Alice and Bob is to return an independent set $R$ of submodular value $f(R)$ as large as possible, while using only a small message size $|Q|$. In particular, we are interested in the achievable trade-offs between the message size $|Q|$ and the approximation guarantee $f(R)/f(\OPT)$ of the returned set $R$, where $\OPT\in \argmax\{f(I) \colon I\in \mathcal{I}\}$ is an optimal solution to the (offline) problem.

In one extreme, Alice can send all of her elements $Q=\cN_A$ to Bob, who can then find (in exponential time) and return an independent set $I\subseteq \cN$ with $f(I) = f(\OPT)$. In the other extreme, one can observe that a message size of $\Omega(k)$ is required to be able to obtain a constant approximation guarantee. In particular, a trivial $\sfrac{1}{2}$-approximation is obtained by Alice sending a maximizer $Q$ of $\max\{f(I)\colon I\in \mathcal{I}, I\subseteq \cN_A\}$ to Bob. To obtain a $\sfrac{1}{2}$-guarantee, it suffices for Bob to return the better of $Q$ and a maximizer of $\max\{f(I) \colon I\in \mathcal{I}, I\subseteq \cN_B\}$.

The result we show in this section is that one can beat the factor of $\sfrac{1}{2}$ with a linear message size.

\thmTwoplayer*

\subsection{The protocol}

We now describe the protocol claimed by \cref{thm:beatHalfForTwoPlayers}. A key step of our protocol is the use of a continuous greedy algorithm for submodular maximization similar to the ones often used to approximately maximize a submodular function under various constraints. It is well-known that such continuous greedy procedures can be discretized to obtain efficient implementations with an arbitrarily small constant loss in the approximation guarantee compared to their continuous counterparts. However, a straightforward discretization would lead to a message size of $O(k^2)$ in our case. We use a discretized version developed by \textcite{badanidiyuru2014fast}, whose goal was to create a very fast algorithm to approximately maximize a non-negative monotone submodular function over a matroid constraint. Even though our focus is not on running time, the method developed in~\cite{badanidiyuru2014fast} has a key property that we can exploit in our context, namely that the procedure returns a fractional point of linear support. The way we employ the algorithm, this linear support condition translates into a linear message size sent from Alice to Bob.


We start by describing the discretized version of the continuous greedy process that Alice will use in our protocol, which is a minor variation of an algorithm presented in~\cite{badanidiyuru2014fast}. The algorithm is shown below as \cref{alg:contGreedy}, where $F\colon[0,1]^\cN\to \mathbb{R}_{\geq 0}$ is the multilinear extension of $f$. Apart from the matroid $M$, given by an independence oracle, the algorithm takes as input a subset $S\subseteq \cN$ and a parameter $h\in \mathbb{Z}_{\geq 1}$. The set $S$ describes the elements of the ground set to which the algorithm is applied. It will later be chosen as $S=\cN_A$ because Alice uses this algorithm in our protocol and can only apply it to the elements she received. The parameter $h$ captures the number of steps in the discretization. Hence, the larger $h$, the better the solution quality. In particular, the larger we choose $h$, the closer is the procedure to being a continuous greedy algorithm. We will later see that $h=125$ is large enough to obtain \cref{thm:beatHalfForTwoPlayers}. Nevertheless, we leave $h$ as a variable to highlight the dependence on $h$ of the obtained approximation guarantee, which explains our choice of $h=125$.

\cref{alg:contGreedy}, being a (discretized version of a) continuous greedy procedure, constructs a point $x$ in the matroid polytope $P_M \coloneqq \{y\in \mathbb{R}^\cN_{\geq 0} \colon y(S) \leq r(S) \;\forall S\subseteq \cN\}$ of $M$, with support in $\cN_A$, i.e., $\supp(x)\coloneqq \{e\in \cN \colon x_e > 0 \}\subseteq \cN_A$. The point $x$ is constructed successively over a constant number of $h$ steps, starting from the zero vector. At each step $i\in [h]$, an independent set $C_i\in \mathcal{I}\cap 2^{\cN_A}$ is constructed, and the final point $x$ is given by $x=\frac{1}{h}\sum_{i=1}^h \characteristic_{C_i}$. Since the sets $C_i$ define the point, and correspond to elements that Alice will pass on to Bob in our protocol, we let the output of \cref{alg:contGreedy} be the sets $C_1,\dots, C_h$ instead of returning the point $x$.

As mention above, \cref{alg:contGreedy} is a slightly modified version of an algorithm due to~\cite{badanidiyuru2014fast}. The most significant difference between the two is that the original algorithm of~\cite{badanidiyuru2014fast} used a thresholding technique on the weights to speed up the step of repeatedly finding an element $u$ at the cost of an additional small error term. However, because running time is not our focus here, we replaced the thresholding by a conceptually simpler step to find $u$. In any case, even our description without thresholding runs in polynomial time, and is therefore not the runtime bottleneck because we also perform steps that require exponential time.\footnote{Instead of constructing the sets $C_i$ in the while loop of \cref{alg:contGreedy} by successively adding elements $u$, one could also choose $C_i\in \argmax\{F(x+\frac{1}{h}\characteristic_{C}) \colon C\in \mathcal{I}\}$. Our analysis would still work out with this choice. However, this would only lead to a very minor simplification of the presentation while turning \cref{alg:contGreedy} into an exponential-time procedure, whereas our version is polynomial-time if we replace the exact computation of $F$ by a strong efficiently computable estimate. This difference is irrelevant for showing \cref{thm:beatHalfForTwoPlayers}, as we anyway design an exponential-time method. Nevertheless, for potential future work, and to better understand where exponential running time is currently needed, it may be helpful to know that sets $C_1,\dots, C_h$ with the desired properties can be computed efficiently.}

\begingroup
\begin{algorithm}
\caption{Discretized version of continuous greedy for matroid constraint}
\label{alg:contGreedy}
\begin{algorithmic}[1]
\Require{Matroid $M=(\cN,\mathcal{I})$, set $S\subseteq \cN$, and $h\in \mathbb{Z}_{\geq 1}$.}
\Ensure{Independent sets $C_1,\dots, C_h\in \mathcal{I}\cap 2^S$.}
\State $x=0 \in \mathbb{R}^\cN$.
\For{$i=1$ \textbf{to} $h$}
  \State $C_i \leftarrow \varnothing$.
  \While{$r(C_i) < r(S)$}
    \State Find $u \in \argmax\left\{F\mleft(x + \frac{1}{h}\cdot \characteristic_{C_i\cup \{e\}}\mright) \colon e\in S \text{ with } C_i\cup \{e\}\in \mathcal{I}\right\}$.
    \State $C_i \leftarrow C_i \cup \{u\}$.
  \EndWhile
  \State $x \leftarrow x + \frac{1}{h} \cdot \characteristic_{C_i}$.
\EndFor
\State \Return{$C_1,\dots, C_h$}.
\end{algorithmic}
\end{algorithm}
\endgroup

Our protocol to obtain \cref{thm:beatHalfForTwoPlayers} is described in \cref{alg:beatHalfForTwoPlayers}.

\begingroup
%\floatname{algorithm}{Protocol}
\begin{algorithm}
\caption{Protocol leading to \cref{thm:beatHalfForTwoPlayers}}
\label{alg:beatHalfForTwoPlayers}

\smallskip
\emph{Alice's protocol}

\begin{algorithmic}[1]

\State Determine $\OPT(\cN_A)\in \argmax\left\{f(I)\colon I\in \mathcal{I}, I\subseteq \cN_A\right\}$.

\State Apply \cref{alg:contGreedy} to $M$ with $S=\cN_A$ and $h=125$ to obtain $C_1,\dots, C_h\in \mathcal{I}\cap 2^{\cN_A}$, and let $x\coloneqq \frac{1}{h}\sum_{i=1}^h \characteristic_{C_i}$.

\State Compute $W \in \argmax\left\{F\left(x \vee \characteristic_H\right)\colon H\in \mathcal{I}, H\subseteq \cN_A\right\}$.

\State Send the elements $Q\coloneqq \OPT(\cN_A) \cup W \cup \bigcup_{i=1}^h C_i$ to Bob.

\end{algorithmic}

\medskip

\emph{Bob's protocol}
\begin{algorithmic}[1]
\State \Return{$R\in \argmax\left\{f(S) \colon S\in \mathcal{I}, S\subseteq Q\cup \cN_B \right\}$}.
\end{algorithmic}

\end{algorithm}
\endgroup




\subsection{Analysis of \texorpdfstring{\cref{alg:beatHalfForTwoPlayers}}{Algorithm~\ref{alg:beatHalfForTwoPlayers}} (proof of \texorpdfstring{\cref{thm:beatHalfForTwoPlayers}}{Theorem~\ref{thm:beatHalfForTwoPlayers}})}

To analyze \cref{alg:beatHalfForTwoPlayers}, we start by introducing some key terminology and notation used throughout our analysis in \cref{sec:twoPlayerTerminology}. Then, before going into technical details, we present in \cref{sec:twoPlayerProofOutline} a thorough outline of the analysis and provide intuition for the proof strategy that leads to the claimed performance guarantee. Finally, in \cref{sec:twoPlayerFormalProof}, we fill in all technical details to obtain a full formal proof of the performance guarantee of \cref{alg:beatHalfForTwoPlayers}.


\subsubsection{Terminology and notation}\label{sec:twoPlayerTerminology}

To show that the set $R$ returned by \cref{alg:beatHalfForTwoPlayers} is a $0.505$-approximation, we define
\begin{equation}\label{eq:defDelta}
\Delta \coloneqq \frac{f(R)}{f(\OPT)}-\frac{1}{2}
\end{equation}
and show that $\Delta \geq 0.005$.

To show that there exists an independent set in $Q\cup \cN_B$ with large value, we consider different candidate solutions that Bob can return in our analysis. To this end, it is often useful to consider candidate solutions that use part of an optimal solution. As previously mentioned, let $\OPT\in \argmax\{f(I)\colon I \in \mathcal{I}\}$ be an arbitrary fixed optimal solution, and we define
\begin{align*}
\OPT_A &\coloneqq \OPT \cap \cN_A\enspace,\text{ and}\\
\OPT_B &\coloneqq \OPT \cap \cN_B\enspace. 
\end{align*}
%
Note that elements of $\OPT_B$ are among those that Bob can return, whereas the elements of $\OPT_A$ are, in general, not part of the set $Q\cup \cN_B$ of elements from which Bob selects a set $R$ to return.


To create candidate solutions by mixing elements from independent sets we encounter in our protocol with elements of $\OPT$---in particular, $\OPT_B$---we heavily rely on the following well-known exchange theorem of matroids.
%
\begin{theorem}[\cite{brylawski_1973_properties,greene_1973_multiple,woodall_1974_exchange}]\label{thm:matBlockExchange}
Let $M=(\cN,\mathcal{I})$ be a matroid, $I,J\in \mathcal{I}$, and let $I_1, I_2$ be a partition of $I$. Then there is a partition $J_1, J_2$ of $J$ such that the following holds simultaneously:
\begin{enumerate}[nosep, label=(\roman*)]
\item $I_1\cup J_2\in \mathcal{I}$, and
\item $I_2\cup J_1\in \mathcal{I}$.
\end{enumerate}
\end{theorem}
%
We start by using the above exchange theorem to split the vector $x = \frac{1}{h}\sum_{i=1}^h \characteristic_{C_i}$, which we get through the discretized continuous greedy algorithm, into two parts $x_A$ and $x_B$ as follows.
Applying \cref{thm:matBlockExchange} to $\OPT$ with partition $\OPT_A, \OPT_B$, and the set $C_i$, we obtain that for every $i\in [h]$ there is a partition of $C_i$ into $C_{i,A}, C_{i,B}$ such that
\begin{enumerate*}[label=(\roman*)]
\item $\OPT_A \cup C_{i,B} \in \mathcal{I}$, and
\item $\OPT_B \cup C_{i,A} \in \mathcal{I}$.
\end{enumerate*}
%
We split the vector $x$ into $x = x_A + x_B$ as follows
\begin{align*}
x_A &\coloneqq \frac{1}{h} \sum_{i=1}^h \characteristic_{C_{i,A}}\enspace,\text{ and}\\
x_B &\coloneqq \frac{1}{h} \sum_{i=1}^h \characteristic_{C_{i,B}}\enspace.
\end{align*}
%
Moreover, for $i\in [h]$, we denote by
\begin{align*}
x^i_B &\coloneqq \frac{1}{h} \sum_{j=1}^i \characteristic_{C_{j,B}}\enspace, \text{ and}\\
x^i_A &\coloneqq \frac{1}{h} \sum_{j=1}^i \characteristic_{C_{j,A}}\enspace,
\end{align*}
a decomposition $x^i = x^i_A + x^i_B$ of the intermediate solution $x^i=\frac{1}{h}\sum_{j=1}^i \characteristic_{C_j}$ obtained in the discretized continuous greedy algorithm after $i$ iterations. By convention, we set $x^0$, $x^0_A$, and $x^0_B$ to be the zero vector in $\mathbb{R}^\cN$, which corresponds to the fact that the discretized continuous greedy algorithm starts with the zero vector. Note that $x^h=x$.

Instead of showing that there are good candidate independent sets within the elements $Q\cup \cN_B$ among which Bob selects a solution, it is often more convenient to show that there is a fractional point $y$ with $\supp(y)\subseteq Q\cup \cN_B$ in the matroid polytope $y\in P_M$ of high multilinear extension value $F(y)$. This approach is sound because it is well-known that the problem of maximizing the multilinear extension on a matroid has no integrality gap (see~\cite{calinescu2011maximizing}).
%
\begin{lemma}\label{lem:losslessRounding}
Let $y\in P_M$. Then there is a set $I\subseteq \mathcal{I}$ with $I \subseteq \supp(y)$ such that $f(I) \geq F(y)$.
\end{lemma}
%
Consequently, Bob returns a set $R$ with $f(R)\geq F(y)$ for any point $y\in P_M$ with $\supp(y)\subseteq Q\cup \cN_B$.


\subsubsection{Outline of analysis and intuition}\label{sec:twoPlayerProofOutline}

To build up intuition, we suggest to think of the special case where $f\colon 2^\cN\to \mathbb{R}_{\geq 0}$ is a coverage function. More precisely, in this case there is a finite universe $U$ and, to every $e \in \cN$, a set $U_e\subseteq U$ is associated. The value of the function $f$ evaluated at some set $S\subseteq \cN$ is then given by $f(S) = | \cup_{e\in S} U_e |$. For simplicity, let us use the shorthand notation $U_S\coloneqq \cup_{e\in S} U_e$ for any $S\subseteq \cN$. Hence, $f(S) = |U_S|$.
Moreover, we suggest to think of the case $f(\cN) = f(\OPT)$. In words, $U_\OPT = U$, i.e., $\OPT$ covers the whole universe.
These suggested assumptions are only to simplify the understanding of the proof plan and main ideas, and are never used in any of our statements or proof.


We now argue why there is no instance for which \cref{alg:beatHalfForTwoPlayers} has an approximation factor arbitrarily close to $\sfrac{1}{2}$. Hence, equivalently, $\Delta$ must be bounded away from zero. First, to obtain an instance for which $\Delta$ may be very small, we claim that both $f(\OPT_A)$ and $f(\OPT_B)$ need to be very close to $\frac{1}{2}f(\OPT)$. Indeed, by submodularity and non-negativity of $f$, we have $f(\OPT) \leq f(\OPT_A) + f(\OPT_B)$. If either $f(\OPT_A)$ or $f(\OPT_B)$ is larger than $\frac{1}{2}f(\OPT)$ by some global constant, then we are done, because Bob has $\OPT(\cN_A)$ and $\OPT_B$ as candidate sets to return and $f(\OPT(\cN_A))\geq f(\OPT_A)$. Hence, a bad instance needs to be such that $\OPT_A$ and $\OPT_B$ cover roughly half of the universe $U$. The above reasoning also implies that they cannot overlap by much. Assume for simplicity that the universe $U$ is partitioned into two equally-sized sets $U_{\OPT_A}$ and $U_{\OPT_B}$; hence, $U_{\OPT_A}$ is fully covered by $\OPT_A$ and $U_{\OPT_B}$ by $\OPT_B$.


Let us now consider the point $x$ we build through \cref{alg:contGreedy}, the discretized continuous greedy procedure, and how a bad instance needs to look like such that the elements of $\supp(x)$ together with $\OPT(\cN_A)$ and $\cN_B$ do not contain an independent set of high value. First, one can show that the three vectors $x_A\vee \characteristic_{\OPT_B}$, $x_B\vee \characteristic_{\OPT_A}$, and $x$ are all in the matroid polytope $P_M$. By \cref{lem:losslessRounding}, this allows us to obtain the following. (Full proof of this and further statements in this subsection are provided in \cref{sec:twoPlayerFormalProof}.)
%
\begin{restatable}[label=obs:boundMixedSols]{observation}{boundMixedSols}
\leavevmode
\begin{enumerate}[nosep, parsep=0.2em, label=(\roman*)]
\item\label{item:combXA} $F\left(x_A \vee \characteristic_{\OPT_B}\right) \leq \left(\frac{1}{2} + \Delta\right)\cdot f(\OPT)$.
\item\label{item:combXB} $F\left(x_B \vee \characteristic_{\OPT_A}\right) \leq \left(\frac{1}{2} + \Delta\right)\cdot f(\OPT)$.
\item\label{item:xValNotHigh} $F(x) \leq \left(\frac{1}{2} + \Delta\right)\cdot f(\OPT)$.
\end{enumerate}
\end{restatable}
%
Indeed, \cref{item:combXA} and \cref{item:xValNotHigh} are immediate consequences of \cref{lem:losslessRounding} and the fact that the support of both $x_A \vee \characteristic_{\OPT_B}$ and $x$ are contained in the elements $Q\cup \cN_B$ among which Bob chooses the independent set of largest submodular value. Moreover, \cref{item:combXB} also follows from \cref{lem:losslessRounding} and the fact that $\supp(x_B\vee \OPT_A)\subseteq \cN_A$, which implies that $f(\OPT(\cN_A)) \geq F(x_B \vee \OPT_A)$. Again, $\OPT(\cN_A)$ is a set that can be returned by Bob because $\OPT(\cN_A)\subseteq Q$.


Hence, interpreting this in our example of a coverage function, we have that, in a bad instance (one with very small $\Delta$), the sets $C_{i,A}$ used to build $x_A$ almost only cover elements of $U_{\OPT_B}$. Analogously, the sets $C_{i,B}$ to build $x_B$ almost only cover elements of $U_{\OPT_A}$.
This has several consequences. In particular, what $x_A$ or $x_B$ ``covers'' has almost no overlap. Hence, $F(x)$ is close to $F(x_A) + F(x_B)$.

Another, more important consequence is that the point $x$ we get through the discretized continuous greedy procedure leads to a high value $F(x)$. More precisely, recall that the discretized continuous greedy algorithm is run by Alice, and is thus only applied to the elements in $\cN_A$. It could be that $f(\cN_A)$ is very close to $\frac{1}{2}f(\OPT)$. Hence, by using a greedy approach, one would normally expect to lose a factor of $1-\sfrac{1}{e}$, which would lead to a lower bound on $F(x)$ of only about $\frac{1}{2}(1-\sfrac{1}{e})f(\OPT)$. However, we can show that $F(x)$ is at least about $\frac{1}{2}f(\OPT)$ for small $\Delta$. The reason for this is the following. Consider an arbitrary iteration $i\in [h]$ of \cref{alg:contGreedy}, and let us use again the special case of a coverage function to better exemplify things. The elements in $\OPT_A$ where candidates to build up the sets $C_{i,A}$ that the discretized continuous greedy chose. As discussed, $\OPT_A$ covers $U_{\OPT_A}$, which is half of the universe. Part of $U_{\OPT_A}$ may already be fractionally covered by $x^{i-1} = x_A^{i-1} + x_B^{i-1}$. However, as mentioned, we can assume (for very small $\Delta$) that only $x_B^{i-1}$ (fractionally) covers elements of $U_{\OPT_A}$. Hence, the marginal contribution of $\OPT_A$ at step $i$ of  \cref{alg:contGreedy} is about $(\frac{1}{2} - F(x_B^{i-1}))f(\OPT)$. Formalizing these arguments leads to the following.
%
\begin{restatable}[label=lem:xAAndxBAverageIsGood]{lemma}{xAAndxBAverageIsGood}
\begin{equation*}
F(x_A) + \frac{1}{h} \sum_{i=1}^h F(x_B^i) \geq \left(\frac{1}{2} - \Delta\right)f(\OPT)\enspace.
\end{equation*}
\end{restatable}
%
Note that \cref{lem:xAAndxBAverageIsGood} indeed implies that $F(x)$ has a value that cannot be far below $\frac{1}{2}f(\OPT)$ for small $\Delta$ because of the following. By monotonicity of $f$, which implies monotonicity of $F$, we have $F(x_B^i) \leq F(x_B)$ for $i\in [h]$. Together with \cref{lem:xAAndxBAverageIsGood} this implies 
$F(x_A) + F(x_B) \geq \left( \frac{1}{2} - \Delta\right)f(\OPT)$.
Finally, we recall that $F(x)$ is close to $F(x_A) + F(x_B)$ because $x_A$ and $x_B$ cover different parts of the universe.

\cref{lem:xAAndxBAverageIsGood} has another interesting consequence. Namely, if we have a bad instance where $F(x_B)$ is bounded away from zero, then $F(x_B)$ must be close to $\frac{1}{h}\sum_{i=1}^h F(x_B^i)$. For otherwise, replacing the term $\frac{1}{h}\sum_{i=1}^h F(x_B^i)$ by $F(x_B)$ in \cref{lem:xAAndxBAverageIsGood} would lead to a significant increase of the left-hand side in \cref{lem:xAAndxBAverageIsGood}, thus showing that $F(x_A) + F(x_B)$ (which is close to $F(x)$) has value strictly above $\sfrac{1}{2}$.
%
Formally, this relation is captured by the following statement.
%
\begin{restatable}[label=lem:averageXBIsCloseToXB]{lemma}{averageXBIsCloseToXB}
\begin{equation*}
\frac{1}{h} \sum_{i=1}^h F(x_B^i) \geq F(x_B) -4\Delta\cdot f(\OPT)\enspace.
\end{equation*}
\end{restatable}
%
\cref{lem:averageXBIsCloseToXB} implies that if $F(x_B)$ is large, then the sequence $F(x_B^1), F(x_B^2), \ldots, F(x^h_B) = F(x_B)$ increases quickly early on. In other words, even for a relatively small index $i^*\in [h]$, we have that $F(x_B^{i^*})$ is close to $F(x_B)$. In case $F(x_B)$ is large, we consider such an index $i^*$ and the point $z\coloneqq x_B^{i^*} + (1-\frac{i^*}{h})\characteristic_{\OPT_B}$, which lies in $P_M$ and whose support is contained in the elements among which Bob chooses a set to return. Because $x_B$, and thus also $x_B^{i^*}$, almost exclusively covers elements in $U_{\OPT_A}$, and $\OPT_B$ is covered by the elements in $U_{\OPT_B}$, we have that $F(z)$ is very close to $F(x_B^{i^*}) + (1-\frac{i^*}{h})f(\OPT_B)$. Hence, if $F(x_B)$ is large, then so is $F(x_B^{i^*})$, and $F(z)$ will be bounded away from $\frac{1}{2}f(\OPT)$ as desired.

Hence, it remains to deal with the case where $F(x_B)$ is small. This is where we rely on the set $W$ that Alice passes to Bob, which we have not used so far. We again crucially exploit that $x$ was constructed with a (discretized version of a) continuous greedy algorithm. Because $F(x_B)$ is small, we have that $F(x_A)$ must be close to $\frac{1}{2}f(\OPT)$ due to \cref{lem:xAAndxBAverageIsGood}. Hence, in the context of our example based on $f$ being a coverage function, this implies that $x_A$ (fractionally) covers almost all of $U_{\OPT_B}$ whereas $U_{\OPT_A}$ remains nearly uncovered. This motivates our choice of $W$ as a maximizer of
\begin{equation}\label{eq:maximizationForW}
\max\left\{F(x\vee \characteristic_H)\colon H\in \mathcal{I}, H\subseteq \cN_A\right\}\enspace.
\end{equation}
Indeed, because it remains to cover $U_{\OPT_A}$, the set $W=\OPT_A$ would be a near maximizer of \cref{eq:maximizationForW}. Of course, $W=\OPT_A$ would be ideal, in which case Bob could even return $\OPT$. In general, $W\subseteq \cN_A$ will be some set that covers nearly all of $U_{\OPT_A}$ but may not overlap with $\OPT_A$. We use \cref{thm:matBlockExchange} to partition $W$ into $W_A$ and $W_B$ such that $W_A\cup \OPT_B\in \mathcal{I}$ and $W_B \cup \OPT_A\in \mathcal{I}$. We want to show that $W_A$ covers a significant fraction of $U_{\OPT_A}$, in which case we are done because Bob can return $W_A\cup \OPT_B$. Hence, the only bad case is if $U_{\OPT_A}$ is almost entirely covered by $W_B$. We argue that, in this case, the discretized version of the continuous greedy algorithm would already have returned a point $x$ with $F(x)$ significantly larger than $\frac{1}{2}f(\OPT)$. The reason is that $\OPT_A\cup W_B$ was a candidate set for each of the sets $C_i$ considered in \cref{alg:contGreedy}. This set nearly ``double-covers'' the almost uncovered part $U_{\OPT_A}$ of the universe. Now we exploit a crucial property of the (discretized) continuous greedy algorithm, namely that its local improvement is given by the sum of the coverages of the elements that get added. In other words, the double coverage of part of the universe of value $\frac{1}{2}f(\OPT)$ also leads to a double contribution to the local improvement, i.e., the gradient would be about $f(\OPT)$. This would have been true for all steps of the discretized continuous greedy algorithm, leading to $F(x)$ being close to $f(\OPT)$ if both $F(x_B)$ and $\Delta$ are small. However, this shows that it is impossible for both $F(x_B)$ and $\Delta$ to be very small when $x$ covers only about half of the universe $U$. Hence, this case is impossible, showing that, if both $F(x_B)$ and $\Delta$ are small, then $f(W_A\cup \OPT_B)$ will be significantly larger than $\frac{1}{2}f(\OPT)$.
%
The statement below quantifies this relationship.
%
\begin{restatable}[label=lem:OptBWALowerBound]{lemma}{OptBWALowerBound}
$f(W_A \cup \OPT_B) \geq (1-4\Delta)f(\OPT) - 3 F(x_B)$.
\end{restatable}

Using that $W_A\cup \OPT_B$ is a set that Bob can return, and must therefore have a value of at most $(\frac{1}{2}+\Delta)f(\OPT)$, we can quantify the fact that not both $F(x_B)$ and $\Delta$ can be very small simultaneously as follows.
%
\begin{restatable}[label=lem:xBLowerBound]{lemma}{xBLowerBound}
$F(x_B) \geq \left(\frac{1}{6} - \frac{5}{3}\Delta\right)\cdot f(\OPT)$.
\end{restatable}

Hence, we finally obtain that it is impossible for both $F(x_B)$ and $\Delta$ to be very small, which brings us back to the case of large $F(x_B)$, for which we have already explained why our protocol obtains an approximation factor that is by some constant larger than $\sfrac{1}{2}$. Putting everything together leads to our claimed lower bound on $\Delta$.
%
\begin{restatable}{theorem}{lowerBoundDelta}
$\Delta \geq 0.005$.
\end{restatable}

\subsubsection{Formal proofs}\label{sec:twoPlayerFormalProof}

We now fill in the details of the previously outlined analysis plan and provide proofs of the mentioned statements. We start by highlighting some basic properties of the multilinear extension $F$.
%
\begin{lemma}[see~\cite{calinescu2011maximizing}]\label{lem:FConcaveNonneg}
Let $f: 2^\cN \to \mathbb{R}_{\geq 0}$ be a submodular function and $F: [0,1]^\cN \to \mathbb{R}_{\geq 0}$ its multilinear extension. Then the following holds.
\begin{enumerate}[label=(\roman*)]
\item For any $x\in [0,1]^\cN$, all entries of the Hessian $\nabla^2 F(x)$ are non-positive. This implies in particular that $F$ is concave along non-negative directions; hence
\begin{equation*}
F(y + \lambda z) \geq (1-\lambda)F(y) + \lambda F(y+z) \qquad \forall y\in [0,1]^\cN, z\in \mathbb{R}^\cN_{\geq 0}, \lambda \in [0,1] \text{ with } y+z\in[0,1]^\cN \enspace.
\end{equation*}

\item If $f$ is monotone then so is $F$, i.e.,
\begin{equation*}
F(y) \leq F(z) \qquad y,z\in [0,1]^\cN \text{ with } y\leq z\enspace.
\end{equation*}
\end{enumerate}
\end{lemma}

The above properties allow for generalizing the diminishing returns property and further properties of submodular functions to the multilinear extensions, as stated in \cref{lem:FSubmodularity} below. The properties listed in \cref{lem:FSubmodularity} readily follow from prior work. (For example, \cref{item:FVeeWedgeSubmod} and \cref{item:FDimReturns} are special cases of~\cite[Lemma~3.11]{chekuri_2014_submodular}, and \cref{item:FVeeWedgeDimReturns} is an immediate consequence of \cref{item:FVeeWedgeSubmod} and the monotonicity of $F$.) Nevertheless, we provide a proof of \cref{lem:FSubmodularity} for completeness. For two vectors $x,y\in \mathbb{R}^\cN$, we use the notation $x \vee y$ for the component-wise maximum of $x$ and $y$, and $x\wedge y$ for their component-wise minimum.
%
\begin{lemma}\label{lem:FSubmodularity}
Let $f:2^\cN\to \mathbb{R}_{\geq 0}$ be a submodular function and $F:[0,1]^\cN\to \mathbb{R}_{\geq 0}$ its multilinear extension. Then the following holds.
\leavevmode
\begin{enumerate}[label=(\roman*),parsep=0.0em,topsep=0.2em]
\item\label{item:FDimReturns} \makebox[6.3cm][l]{$F(w+y) - F(y) \geq F(w+z) - F(z)$} $\forall w,y,z\in [0,1]^\cN$ with $y\leq z$ and $w+z\in [0,1]^\cN$\enspace.
\item\label{item:FVeeWedgeSubmod} \makebox[6.3cm][l]{$F(w) + F(y) \geq F(w \vee y) + F(w\wedge y)$} $\forall w,y\in [0,1]^\cN$\enspace.
\item\label{item:FVeeWedgeDimReturns} Moreover, if $f$ is monotone, then\\
\makebox[6.3cm][l]{$F(w\vee y) - F(y) \geq F(w\vee z) - F(z)$} $\forall w,y,z\in [0,1]^\cN$ with $y\leq z$\enspace.
\end{enumerate}
\end{lemma}
%
\begin{proof}
We start by proving \cref{item:FDimReturns}, which follows readily from the non-positivity of the Hessian of $F$:
\begin{align*}
F(w + z) - F(z) - (F(w + y) - F(y))
  &= \int_0^1 w^T \left(\nabla F(z + tw) - \nabla F(y+tw)\right)\, dt     \\
  &= \int_0^1 \int_0^1 w^T \nabla^2 F(y + tw + \tau(z-y))(z-y)\,d\tau\,dt \\
  &\leq 0\enspace,
\end{align*}
where the inequality follows from $w\geq 0$, $z-y\geq 0$, and $\nabla^2 F(y + tw + \tau(z-y)) \leq 0$.


\cref{item:FVeeWedgeSubmod} follows from \cref{item:FDimReturns} because
\begin{align*}
F(w\vee y) - F(w) &= F\left(w + ((w\vee y) - w)\right) - F(w)         \\
                  &\geq F((w\wedge y) + ((w\vee y)-w)) - F(w\wedge y) \\
                  &=F(y) - F(w\wedge y)\enspace,
\end{align*}
where the second inequality is due to \cref{item:FDimReturns} and the last one uses $(w\wedge y) + (w\vee y) = w + y$.

Finally, \cref{item:FVeeWedgeDimReturns} can be derived from \cref{item:FVeeWedgeSubmod} and the monotonicity of $F$ as follows.
\begin{align*}
F(w\vee y) + F(z) &\geq F((w\vee y) \vee z) + F((w\vee y)\wedge z) \\
                  &\geq F(w\vee z) + F(y)\enspace,
\end{align*}
where the first inequality is due to \cref{item:FVeeWedgeSubmod}, and the second one follows from $(w\vee y) \vee z = w\vee z$, which holds because $z\geq y$, and $F((w\vee y) \wedge z) \geq F(y)$, which holds because $(w\vee y) \wedge z \geq y$ (again, using $z\geq y)$ and $F$ is monotone.
\end{proof}


Using these properties of the multilinear extension, we are now ready to provide a formal proof of \cref{obs:boundMixedSols}.
\boundMixedSols*
%
\begin{proof}
\cref{item:combXA}: We first observe that $x_A\vee\characteristic_{\OPT_B}\in P_M$ because
\begin{align*}
x_A \vee \characteristic_{\OPT_B} &= \left(\frac{1}{h}\sum_{i=1}^h \characteristic_{C_{i,A}}\right) \vee \characteristic_{\OPT_B}\\
%                      
                       &= \frac{1}{h}\sum_{i=1}^h \left(\characteristic_{C_{i,A}} \vee \characteristic_{\OPT_B}\right)\\
%
                       &= \frac{1}{h}\sum_{i=1}^h \characteristic_{C_{i,A}\cup \OPT_B}\enspace,
\end{align*}
which shows that $x_A \vee \characteristic_{\OPT_B}$ is a convex combination of the points $\characteristic_{C_{i,A}\cup \OPT_B}$ for $i\in [h]$; moreover, $\characteristic_{C_{i,A}\cup \OPT_B}\in P_M$, because $C_{i,A}\cup \OPT_B\in \mathcal{I}$. Furthermore, $\supp(x_A \vee \characteristic_{\OPT_B})\subseteq Q \cup \cN_B$, and $Q\cup \cN_B$ are the elements among which Bob chooses the largest-valued independent set $R$ to return. The statement now follows by \cref{lem:losslessRounding}, which implies $f(R) \geq F(x_A \vee \characteristic_{\OPT_B})$, and the definition of $\Delta$ (see \cref{eq:defDelta}).

\cref{item:combXB} The proof of this statement is identical to the proof of \cref{item:combXA} with the roles of $A$ and $B$ exchanged.


\cref{item:xValNotHigh}: By construction, $x = \frac{1}{h}\sum_{i=1}^h \characteristic_{C_i}$ is a point in the matroid polytope $P_M$, because $C_i\in \mathcal{I}$ for $i\in [h]$, and its support is contained in $Q$. Hence, as before, the statement follows by \cref{lem:losslessRounding}.
\end{proof}

As mentioned, \cref{obs:boundMixedSols} can be interpreted, in the context of $f$ being a coverage function, as stating that $x_A$ heavily overlaps with $\OPT_B$ and, analogously, $x_B$ heavily overlaps with $\OPT_A$, in terms of what parts of the universe they cover. Another way to phrase this is that $x_A$ has little overlap with $\OPT_A$ and, analogously, $x_B$ has little overlap with $\OPT_B$. These relations, stated formally below, are in some circumstances more convenient.
%
\begin{lemma}\label{lem:boundNonMixedSols}
\leavevmode
\begin{enumerate}[nosep, parsep=0.2em, label=(\roman*)]
\item\label{item:xAWithOptA} $F(x_A \vee \characteristic_{\OPT_A}) \geq \left(\frac{1}{2} - \Delta\right)\cdot f(\OPT) + F(x_A)$.
\item\label{item:xBWithOptB} $F(x_B \vee \characteristic_{\OPT_B}) \geq \left(\frac{1}{2} - \Delta\right)\cdot f(\OPT) + F(x_B)$.
\end{enumerate}
\end{lemma}
%
\begin{proof}
We only prove the first statement. The proof of the second one is identical with the roles of $A$ and $B$ exchanged.
\begin{align*}
F\left(x_A \vee \characteristic_{\OPT_A}\right) &= F\left(x_A \vee \characteristic_{\OPT_A}\right) - F(x_A) + F(x_A) \\
                                                &\geq F\left(x_A \vee \characteristic_{\OPT_A \cup \OPT_B}\right) - F\left(x_A \vee \characteristic_{\OPT_B}\right) + F(x_A) \\
                                                &\geq f(\OPT) - \left(\frac{1}{2} + \Delta\right)f(\OPT) + F(x_A) \\
                                                &= \left( \frac{1}{2} - \Delta \right) f(\OPT) + F(x_A)\enspace,
\end{align*}
where the first inequality follows from \cref{item:FVeeWedgeDimReturns} of \cref{lem:FSubmodularity}   and the second one follows from \cref{lem:boundNonMixedSols} and $F(x_A\vee \characteristic_{\OPT_A \cup \OPT_B}) \geq F(\characteristic_{\OPT}) = f(\OPT)$, which holds due to monotonicity of $F$.
\end{proof}


As previously discussed, $x_A$ and $x_B$ have little overlap, which implies that $F(x_A) + F(x_B)$ is close to $F(x)$. In turn, $F(x)$ is no larger than 
$(\frac{1}{2} + \Delta)f(\OPT)$ because of \cref{lem:losslessRounding}. Combining and formalizing these statements leads to the following result.
%
\begin{lemma}\label{lem:boundFxAAndFxB}
$F(x_A) + F(x_B) \leq \left(\frac{1}{2} + 3\Delta\right)\cdot f(\OPT)$.
\end{lemma}
%
\begin{proof}
We have
\begin{align*}
\left(\frac{1}{2} + \Delta\right)\cdot f(\OPT) &\geq F(x) \\
                                               &=    F(x_A) + F(x) - F(x_A)\\
                                               &\geq F(x_A) + F\left(x\vee \characteristic_{\OPT_B}\right) - F\left(x_A\vee\characteristic_{\OPT_B}\right)\\
                                               &\geq F(x_A) + F\left(x_B \vee \characteristic_{\OPT_B}\right) - F\left(x_A \vee \characteristic_{\OPT_B}\right)\\
                                               &\geq F(x_A) + F(x_B) - 2\Delta\cdot f(\OPT) \enspace,
\end{align*}
where the first inequality follows by \cref{item:FVeeWedgeDimReturns} of \cref{lem:FSubmodularity}, the second one by monotonicity of $F$, and the last one by \cref{item:xBWithOptB} of \cref{lem:boundNonMixedSols}~ and by \cref{item:combXA} of \cref{obs:boundMixedSols}. The claimed result follows by reordering terms.
\end{proof}


We now start to analyze properties of the discretized continuous greedy procedure, i.e., \cref{alg:contGreedy}. We start by deriving guarantees on the improvement happening in a single iteration. More precisely, the statement below shows that the improvement at some iteration $i$ is at least as good as the best improvement that could have been achieved in the next iteration. This idea and the corresponding proof technique go back to~\textcite{badanidiyuru2014fast}. We provide a full proof in our context for convenience.
%
\begin{lemma}\label{lem:discContGreedyProp}
Let $i\in [h]$ and let $X\subseteq C_i, Y\subseteq \cN_A$ satisfying
\begin{enumerate}[label=(\alph*),parsep=0.2em,topsep=0.2em,itemsep=0.2em]
\item $|X| = |Y|$, and
\item $(C_i \setminus X) \cup Y \in \mathcal{I}$.
\end{enumerate}
Then
\begin{align*}
F\left(x^{i-1} + \frac{1}{h}\characteristic_X\right) - F\left(x^{i-1}\right)
&\geq \sum_{y\in Y} \left[F\left(\left(x^i + \frac{1}{h} \characteristic_{y}\right)\wedge \characteristic_{\cN} \right) - F\left(x^i\right)\right] \\
&\geq \frac{1}{h} \sum_{y\in Y} \left[F\left(x^i \vee \characteristic_{y}\right) - F\left(x^i\right)\right]\enspace.
\end{align*}
%
\end{lemma}
%
\begin{proof}
We start by proving the first inequality.
Let $C_i = \{u_1,\ldots, u_{\rho}\}$, where the numbering corresponds to the order in which elements where added to $C_i$ in the construction of $C_i$ described by \cref{alg:contGreedy}. Let $X=\{u_{j_1}, u_{j_2},\ldots, u_{j_k}\}$ with $j_1,\ldots, j_k\in [\rho]$ and the numbering of the indices is chosen such that $j_1 < j_2 < \ldots < j_k$. Because $|X|=|Y|$ and both $C_i\in \mathcal{I}$ and $(C_i\setminus X)\cup Y \in \mathcal{I}$, classical results in matroid theory guarantee that there is a bijection (often called \emph{Brualdi bijection}) $\phi\colon X\to Y$ such that
\begin{equation*}
(C_i \setminus \{u\}) \cup \{\phi(u)\}\in \mathcal{I} \qquad \forall u \in X\enspace.
\end{equation*}
%
Moreover, we define
\begin{equation*}
\lambda_\ell \coloneqq \min\left\{\frac{1}{h}, 1- x^i(\phi(u_{j_\ell}))\right\} \qquad \forall \ell \in [k]\enspace.
\end{equation*}

The first inequality now follows by the relations below, whose individual steps will be further explained in the following.
\begin{align*}
F\bigg(x^{i-1} &+ \frac{1}{h}\characteristic_X\bigg) - F\left(x^{i-1}\right)\\
%
  &= \sum_{\ell=1}^k \left[F\left(x^{i-1} + \frac{1}{h} \characteristic_{\{u_{j_1},u_{j_2},\ldots, u_{j_\ell}\}} \right) - F\left(x^{i-1} + \frac{1}{h} \characteristic_{\{u_{j_1},u_{j_2},\ldots, u_{j_{\ell-1}}\}}\right) \right]\\
%
  &\geq \sum_{\ell=1}^k \left[ F\left(x^{i-1} + \frac{1}{h} \characteristic_{\{u_1,\ldots, u_{j_\ell}\}}\right) - F\left(x^{i-1} + \frac{1}{h} \characteristic_{\{u_1,\ldots, u_{j_\ell -1}\}}\right) \right]\\
%
  &\geq \sum_{\ell=1}^k \left[ F\left(x^{i-1} + \frac{1}{h} \characteristic_{\{u_1,\ldots, u_{j_\ell - 1}\}} + \frac{1}{h} \characteristic_{\phi(u_{j_\ell})} \right) - F\left(x^{i-1} + \frac{1}{h} \characteristic_{\{u_1,\ldots, u_{j_\ell -1}\}}\right) \right]\\
%
  &\geq \sum_{\ell=1}^k \left[ F\left(x^{i-1} + \frac{1}{h} \characteristic_{\{u_1,\ldots, u_{j_\ell - 1}\}} + \lambda_\ell \cdot \characteristic_{\phi(u_{j_\ell})} \right) - F\left(x^{i-1} + \frac{1}{h} \characteristic_{\{u_1,\ldots, u_{j_\ell -1}\}}\right) \right]\\
%
  &\geq \sum_{\ell=1}^k \left[ F\left(x^i + \lambda_\ell \cdot \characteristic_{\phi(u_{j_\ell})} \right) - F(x^i) \right]\\
%
  &= \sum_{\ell=1}^k \left[ F\left(\left(x^i + \frac{1}{h} \cdot \characteristic_{\phi(u_{j_\ell})}\right)\wedge \characteristic_\cN \right) - F(x^i) \right]\\
%
  &= \sum_{y\in Y} \left[ F\left(\left(x^i + \frac{1}{h} \cdot \characteristic_{y}\right)\wedge \characteristic_\cN \right) - F(x^i) \right]\enspace.
\end{align*}
%
The first inequality holds due to \cref{item:FDimReturns} of \cref{lem:FSubmodularity}.
The second one is a consequence of how the set $C_i=\{u_1,\ldots, u_\rho\}$ was constructed. More precisely, for any $\ell\in [k]$, the element $u_{j_\ell}$ was chosen to be the element $e$ maximizing the expression 
$F(x^{i-1} + \frac{1}{h} \characteristic_{\{u_1,\ldots, u_{j_{\ell-1}}\}\cup\{e\}}) - F(x^{i-1} + \frac{1}{h} \characteristic_{\{u_1,\ldots, u_{j_\ell -1}\}})$ among all elements $e\in \cN_A$ with $\{u_1,\ldots, u_{j_{\ell-1}}\}\cup\{e\}\in \mathcal{I}$. Moreover, $\{u_1,\ldots, u_{j_{\ell-1}}\}\cup \{\phi(u_{j_\ell})\} \subseteq (C_i\setminus \{u_{j_\ell}\})\cup \{\phi(u_{j_\ell})\} \in \mathcal{I}$; hence, $\phi(u_{j_\ell})$ was a candidate element considered when $u_{j_\ell}$ was picked in the construction of $C_i$.
The third inequality follows from $\lambda_\ell \leq \sfrac{1}{h}$ and the monotonicity of $F$.
The fourth inequality is implied by \cref{item:FDimReturns} of \cref{lem:FSubmodularity}.
The penultimate equality is due to the definition of $\lambda_\ell$.
Finally, the last equality holds because $\phi$ is a bijection from $X$ to $Y$.

We now show the second inequality of the statement, which follows by properties of $F$ and holds even for any set $Y\subseteq \cN$. For every $y\in Y$ we have
\begin{align*}
\frac{1}{h} F\left(x^i \vee \characteristic_{y}\right) + \left(1-\frac{1}{h}\right)F\left(x^i\right)
  &\leq F\left(x^i + \frac{1}{h} \left(\left(x^i \vee \characteristic_{y}\right)-x^i\right)\right)    \\
  &= F\left(x^i + \frac{1}{h} \left(1-x^i(y)\right)\characteristic_{y}\right)                           \\
  &\leq F\left(\left(x^i + \frac{1}{h} \characteristic_{y}\right)\wedge \characteristic_{\cN}\right)\enspace,
\end{align*}
%
where the first inequality holds due to concavity of $F$ along non-negative directions (\cref{lem:FConcaveNonneg}), and the second inequality follows by monotonicity of $F$. The above inequality implies
\begin{equation*}
\frac{1}{h}\left(F\left(x^i \vee \characteristic_{y}\right) - F\left(x^i\right)\right) \leq F\left(\left(x^i + \frac{1}{h} \characteristic_{y}\right)\wedge \characteristic_{\cN}\right) - F\left(x^i\right) \qquad \forall y\in Y\enspace,
\end{equation*}
which shows the second inequality of the statement, as desired.
\end{proof}


The statement below, which, as we show, is a consequence of the first inequality of \cref{lem:discContGreedyProp}, shows that the marginal gains of $F(x^i)$ over the iterations of \cref{alg:contGreedy} are non-increasing.

\begin{lemma}\label{lem:margXiNonInc}
\begin{equation*}
F(x^{i+1}) - F(x^i) \leq F(x^i) - F(x^{i-1}) \qquad \forall i \in [h-1]\enspace.
\end{equation*}
\end{lemma}
%
\begin{proof}
We invoke \cref{lem:discContGreedyProp} with $X=C_i$ and $Y=C_{i+1}$. Note that by construction of the sets $C_i$ we have $|C_i| = r(\cN_A) = |C_{i+1}|$. Moreover, $(C_i \setminus X) \cup Y  = C_{i+1} \in \mathcal{I}$. Hence, the conditions of \cref{lem:discContGreedyProp} are satisfied and we have
\begin{equation}\label{eq:FxiMarginalsIneqSplit}
\begin{aligned}
F(x^{i}) - F(x^{i-1}) &= F\left(x^{i-1} + \frac{1}{h}\characteristic_{C_i}\right) - F\left(x^{i-1}\right) \\
&\geq \sum_{y\in C_{i+1}} \left[F\left(\left(x^i + \frac{1}{h} \characteristic_{y}\right)\wedge \characteristic_{\cN} \right) - F\left(x^i\right)\right]\\
&= \sum_{y\in C_{i+1}} \left[F\left(x^i + \frac{1}{h} \characteristic_{y} \right) - F\left(x^i\right)\right]\enspace,
\end{aligned}
\end{equation}
where the inequality follows from \cref{lem:discContGreedyProp} and the second equality from the fact that $x^i \in \frac{i}{h} P_M$ and $i<h$, which implies that each entry of $x^i$ is at most $1-\sfrac{1}{h}$. Moreover, for an arbitrary numbering $C_{i+1}=\{y_1,\ldots, y_p\}$ of the elements in $C_{i+1}$, we have
\begin{align*}
\sum_{y\in C_{i+1}} \left[F\left(x^i + \frac{1}{h} \characteristic_{y} \right) - F\left(x^i\right)\right] 
  &= \sum_{j=1}^p \left[F\left(x^i + \frac{1}{h} \characteristic_{y_j} \right) - F\left(x^i\right)\right] \\
  &\geq \sum_{j=1}^p \left[F\left(x^i + \frac{1}{h} \characteristic_{\{y_1,\ldots,y_j\}} \right) - F\left(x^i + \frac{1}{h}\characteristic_{\{y_1,\ldots, y_{j-1}\}}\right)\right] \\
  &= F\left(x^{i+1}\right) - F\left(x^i\right)\enspace,
\end{align*}
where the inequality follows by \cref{item:FDimReturns} of \cref{lem:FSubmodularity}.
The desired result is obtained by combining the above inequality with \cref{eq:FxiMarginalsIneqSplit}.
\end{proof}


We are now ready to prove \cref{lem:xAAndxBAverageIsGood}.
%
\xAAndxBAverageIsGood*
%
\begin{proof}
For each $i\in [h]$, we have
\begin{align*}
F\left(x^{i-1} + \frac{1}{h} \characteristic_{C_{i,A}} \right) - F(x^{i-1})
 &\geq \frac{1}{h} \left( F \left( x^i \vee \characteristic_{\OPT_A}   \right) -F(x^i)              \right)           \\
 &\geq \frac{1}{h} \left( F \left( x^i \vee \characteristic_{\OPT_A}   \right) - F(x_A^i) -F(x_B^i) \right)           \\
 &\geq \frac{1}{h} \left( F \left( x_A^i \vee \characteristic_{\OPT_A} \right) - F(x_A^i) -F(x_B^i) \right)           \\
 &\geq \frac{1}{h} \left( F \left( x_A \vee \characteristic_{\OPT_A}   \right) - F(x_A) -F(x_B^i)   \right)           \\
 &\geq \frac{1}{h} \left(   \left( \frac{1}{2} - \Delta     \right) f(\OPT) -F(x_B^i)    \right) \enspace, \\
\end{align*}
where the first inequality follows from \cref{lem:discContGreedyProp} with $X=C_{i,A}$ and $Y=\OPT_A$, the second one from \cref{item:FDimReturns} of \cref{lem:FSubmodularity}  with $w = x_A^i$, $z = x_B^i$, and $y=0$ is the zero vector, the third one from monotonicity of $F$, the forth one is a consequence of \cref{item:FVeeWedgeDimReturns} of \cref{lem:FSubmodularity}, and the last one follows from \cref{item:xAWithOptA} of \cref{lem:boundNonMixedSols}.

By summing up both sides of the above inequality over all $i\in [h]$ and reordering terms, we obtain the desired result:
\begin{align*}
\left( \frac{1}{2} - \Delta \right) f(\OPT)
  &\leq \sum_{i=1}^h \left(F\left(x^{i-1} + \frac{1}{h} \characteristic_{C_{i,A}}\right) - F\left(x^{i-1}\right)\right) + \frac{1}{h} \sum_{i=1}^h F\left(x_B^i\right) \\
  &\leq \sum_{i=1}^h \left(F\left(x_A^{i-1} + \frac{1}{h} \characteristic_{C_{i,A}}\right) - F\left(x_A^{i-1}\right)\right) + \frac{1}{h} \sum_{i=1}^h F\left(x_B^i\right) \\
  &=\sum_{i=1}^h \left(F\left(x_A^i\right) - F\left(x_A^{i-1}\right)\right) + \frac{1}{h} \sum_{i=1}^h F\left(x_B^i\right) \\
  &= F(x_A) - f(\varnothing) + \frac{1}{h} \sum_{i=1}^h F\left(x_B^i\right) \\
  &\leq F(x_A) + \frac{1}{h} \sum_{i=1}^h F\left(x_B^i\right)\enspace,
\end{align*}
where the second inequality is due to \cref{item:FDimReturns} of \cref{lem:FSubmodularity} , and the last one follows from $f(\varnothing)\geq 0$.
\end{proof}

\cref{lem:averageXBIsCloseToXB}, which we mentioned in the outline of the analysis, can now readily be derived from \cref{lem:xAAndxBAverageIsGood}.
%
\averageXBIsCloseToXB*
%
\begin{proof}
This results follows from
\begin{align*}
\frac{1}{h}\sum_{i=1}^h F(x_B^i)
  &\geq \left( \frac{1}{2} - \Delta \right)f(\OPT) - F(x_A) \\
  &\geq F(x_B) - 4\Delta f(\OPT)\enspace,
\end{align*}
where the first inequality is due to \cref{lem:xAAndxBAverageIsGood} and the second one is a consequence of \cref{lem:boundFxAAndFxB}.
\end{proof}

We now start to analyze properties of the set $W$ computed by Alice. We recall that we use \cref{thm:matBlockExchange} to partition $W$ into sets $W_A$ and $W_B$ such that $\OPT_A\cup W_B \in \mathcal{I}$ and $\OPT_B\cup W_A \in \mathcal{I}$. We fix one such partition and use it throughout the analysis that follows.
%
In our analysis of $W$, we start by showing that if $F(x_A)$ is close to $\frac{1}{2}f(\OPT)$, and $\Delta$ is small, then $W_B$ largely overlaps with $x$. Indeed, the statement of \cref{lem:xWbUpperBound} implies that in this case $F(x\vee \characteristic_{W_B})$ is close to $\frac{1}{2}f(\OPT)$.
%
\begin{lemma}\label{lem:xWbUpperBound}
\begin{equation*}
F\left(x \vee \characteristic_{W_B}\right) \leq 3 F(x) - F\left(x_A\right) - \left(\frac{1}{2} - \Delta\right)\cdot f(\OPT)\enspace.
\end{equation*}
\end{lemma}
%
\begin{proof}
\cref{lem:discContGreedyProp} allows us to obtain the following lower bound on the marginal improvement of the last iteration, i.e., iteration $h$, of \cref{alg:contGreedy}:
\begin{equation}\label{eq:xWbUBLastStepGood}
\begin{aligned}
F\left(x^h\right) - F\left(x^{h-1}\right)
  &= F\left(x^{h-1} + \frac{1}{h} \characteristic_{C_h}\right) - F\left(x^{h-1}\right)\\
  &\geq \frac{1}{h}\sum_{e\in \OPT_A\cup W_B} \left[F\left(x \vee \characteristic_{e}\right) - F(x) \right]\\
  &\geq \frac{1}{h}\left[F\left(x\vee \characteristic_{\OPT_A}\right) - F(x) + F\left(x\vee \characteristic_{W_B}\right) - F(x)\right]\enspace,
\end{aligned}
\end{equation} 
where the second inequality is implies by the fact that for any set $S\subseteq \cN$, we have $\sum_{e\in S}[F(x \vee \characteristic_{e})-F(x)]\geq F(x\vee \characteristic_S) - F(x)$, which holds because of the following. Let $S=\{e_1,\dots, e_p\}$ be an arbitrary numbering of the elements of $S$. Then
\begin{align*}
\sum_{e\in S} \left[ F\left(x\vee \characteristic_{e}\right) - F(x) \right]
  &= \sum_{i=1}^p \left[ F\left(x\vee \characteristic_{e_i}\right) - F(x) \right]                                    \\
  &\geq \sum_{i=1}^p \left[ F(x\vee \characteristic_{\{e_1,\dots, e_{i}\}}) - F(x\vee \characteristic_{e_1,\dots,e_{i-1}})\right] \\
  &=F(x\vee \characteristic_S) - F(x)\enspace,
\end{align*}
where the inequality follows from \cref{item:FVeeWedgeDimReturns} of \cref{lem:FSubmodularity}.

Moreover, by Lemma \cref{lem:margXiNonInc}, we have for any $i\in [h]$:
\begin{align*}
F(x) - F\left(x^{h-1}\right) &\leq F\left(x^i\right) - F\left(x^{i-1}\right)\enspace.
\end{align*}
%
Combining the above relation with \cref{eq:xWbUBLastStepGood} and summing up over all $i\in [h]$ leads to
\begin{equation}\label{eq:xWbUBSummedOverI}
\begin{aligned}
F(x) - f(\varnothing) &\geq F\left(x\vee \characteristic_{\OPT_A}\right)      -  F(x) + F\left(x\vee \characteristic_{W_B}\right) - F(x)  \\
                      &\geq F\left(x_A \vee \characteristic_{\OPT_A}\right)   -2 F(x) + F\left(x\vee \characteristic_{W_B}\right)\enspace,
\end{aligned}
\end{equation}
where the second inequality is due to monotonicity of $F$. Finally, we lower bound the term $F(x_A \vee \characteristic_{\OPT_A})$ by using \cref{item:xAWithOptA} of  \cref{lem:boundNonMixedSols}~ i.e., 
\begin{align*}
F\left(x_A \vee \characteristic_{\OPT_A}\right) &\geq \left(\frac{1}{2} - \Delta\right)f(\OPT) + F(x_A)\enspace,
\end{align*}
which, after plugging it into \cref{eq:xWbUBSummedOverI}, using $f(\varnothing)\geq 0$, and reordering terms, leads to the desired result.
\end{proof}

We recall that our goal in this part is to show that $f(W_A\cup \OPT_B)$ has a large value if both $\Delta$ and $F(x_B)$ is small (which implies that $F(x_A)$ is large). Our proof plan is to first observe that $F(x\vee \characteristic_W)$ is large, and then show that $W_A$ covers a substantial part of what $\OPT_A$ covers. The lemma below deals with the first part by showing that $F(x \vee \characteristic_W)$ is large if both $F(x_A)$ and $\Delta $ are small.
%
\begin{lemma}\label{lem:xWLowerBound}
\begin{equation*}
F\left(x \vee \characteristic_W\right) \geq \left(\frac{1}{2} - \Delta\right)\cdot f(\OPT) + F(x_A) \enspace.
\end{equation*}
\end{lemma}
\begin{proof}
The statement follows from
\begin{align*}
F\left(x \vee \characteristic_W\right) \geq F\left(x_A \vee \characteristic_{\OPT_A}\right) 
                            \geq \left(\frac{1}{2} - \Delta\right)\cdot f(\OPT) + F(x_A)\enspace,
\end{align*}
where the first inequality follows from monotonicity of $F$ and the second one from \cref{item:xAWithOptA} of \cref{lem:boundNonMixedSols}.
\end{proof}


The next lemma show that, if $F(x_B)$ and $\Delta$ are small, then $W_A$ indeed covers what is not yet covered by $x_A$. Because, if $F(x_B)$ is small, the vector $x_A$ mainly covers what $\OPT_B$ covers, this indeed implies that $W_A$ covers mainly what is covered by $\OPT_A$.
%
\begin{lemma}\label{lem:xaWaLowerBound}
\begin{equation*}
F\left(x_A \vee \characteristic_{W_A}\right) \geq (1 - 2 \Delta)\cdot f(\OPT) - 3 F(x_B) \enspace.
\end{equation*}
\end{lemma}
%
\begin{proof}
By \cref{item:FVeeWedgeDimReturns} of \cref{lem:FSubmodularity}, we have
\begin{equation}\label{eq:xaWaLowerBoundUncross}
F\left(x_A \vee \characteristic_{W_A}\right) - F(x_A)  \geq  F\left(x\vee \characteristic_W\right) - F\left(x \vee \characteristic_{W_B}\right)\enspace.
\end{equation}
Finally, the relation follows from
\begin{align*}
F(x_A \vee \characteristic_{W_A}) &\geq F\left(x\vee \characteristic_W\right) - F\left(x\vee \characteristic_{W_B}\right) + F(x_A)                        \\
                                  &\geq F\left(x\vee \characteristic_W\right) - 3F(x) + 2F(x_A) + \left(\frac{1}{2}-\Delta\right)\cdot f(\OPT) \\
                                  &\geq (1-2\Delta)\cdot f(\OPT)   - 3F(x) + 3F(x_A)                                                \\
                                  &\geq (1-2\Delta)\cdot f(\OPT)   - 3F(x_B) \enspace,
\end{align*}
where the first inequality is due to \cref{eq:xaWaLowerBoundUncross}, the second one follows from \cref{lem:xWbUpperBound}, the third one from \cref{lem:xWLowerBound}, and the last one uses $F(x) \leq F(x_A) + F(x_B)$, which holds due to \cref{item:FVeeWedgeDimReturns} of \cref{lem:FSubmodularity} and $f(\varnothing)\geq 0$.
\end{proof}


Finally, \cref{lem:xWLowerBound} now allows for proving \cref{lem:OptBWALowerBound}, which we stated in the outline of the analysis.
%
\OptBWALowerBound*
%
\begin{proof}
The desired relation follows from
\begin{equation}\label{eq:OptBWALowerBound}
\begin{aligned}
f(W_A \cup \OPT_B) &=    f(W_A \cup \OPT_B) - f(\OPT_B) + f(\OPT_B) \\
                   &\geq F\left(\characteristic_{W_A\cup \OPT_B} \vee x_A\right) - F\left(\characteristic_{\OPT_B} \vee x_A\right) + f(\OPT_B) \\
                   &\geq F\left(\characteristic_{W_A} \vee x_A\right) - F\left(\characteristic_{\OPT_B} \vee x_A\right) + \left(\frac{1}{2}-\Delta\right)f(\OPT) \\
                   &\geq (1-4\Delta) f(\OPT) - 3 F(x_B)\enspace,
\end{aligned}
\end{equation}
where the above-used relations hold due to the following.
The first inequality holds due to \cref{item:FVeeWedgeDimReturns} of \cref{lem:FSubmodularity}.
The second one uses monotonicity of $F$ and $f(\OPT_B)\geq (\sfrac{1}{2} - \Delta)f(\OPT)$, which holds because
\begin{equation*}
f(\OPT_B) \geq f(\OPT) - f(\OPT_A) \geq f(\OPT) - \left(\frac{1}{2} + \Delta\right)f(\OPT) = \left(\frac{1}{2}-\Delta\right)f(\OPT)\enspace,
\end{equation*}
where the first inequality follows by submodularity and non-negativity of $f$, and the second one by $f(\OPT_A)\leq f(R) \leq (\frac{1}{2}+\Delta)f(\OPT)$, because $\OPT_A$ is a candidate set that Bob could return.
Finally, the last inequality of \cref{eq:xBLowerBound} follows by \cref{lem:xaWaLowerBound} and \cref{item:combXA} of \cref{obs:boundMixedSols}. 
\end{proof}


As discussed, as a quite straightforward consequence of \cref{lem:OptBWALowerBound}, we obtain that it is impossible for $F(x_B)$ and $\Delta$ both to be very small.
\xBLowerBound*
%
\begin{proof}
The claimed relation is an immediate consequence of 
\begin{equation}\label{eq:xBLowerBound}
\begin{aligned}
\left(\frac{1}{2} + \Delta\right) f(\OPT) &=    f(R) \\
                                          &\geq f(W_A \cup \OPT_B) \\
                                          &\geq (1-4\Delta) f(\OPT) - 3 F(x_B)\enspace,
\end{aligned}
\end{equation}
where the first inequality follows from the fact that $W_A\cup \OPT_B\in \mathcal{I}$ is a candidate set that Bob could return, and the second one is due to \cref{lem:OptBWALowerBound}.
\end{proof}

By putting everything together, we obtain our main result of this section.
%
\lowerBoundDelta*
%
\begin{proof}
Let $i^*\in [h]$ be a maximizer of $F(x_B^i) - \frac{i}{2h} f(\OPT)$, i.e., 
\begin{align*}
i^*   &\in \argmax\left\{F\left(x_B^i\right) - \frac{i}{2h}f(\OPT) \colon i\in [h]\right\}\enspace, \text{and we define} \\
\beta &\coloneqq F\left(x_B^{i^*}\right) - \frac{i^*}{2h} f(\OPT)\enspace.
\end{align*}
%
Moreover, we define
\begin{equation*}
\gamma\coloneqq \frac{2h(F(x_B)-\beta)}{f(\OPT)}\enspace.
\end{equation*}
We use these quantities to lower bound the term $\frac{1}{h}\sum_{i=1}^h F(x_B^i)$ as follows:
\begin{equation}\label{eq:upperBoundAverageFxBi}
\begin{aligned}
\frac{1}{h} \sum_{i=1}^h F\left(x_B^i\right)
  &\leq \frac{1}{h} \sum_{i=1}^h \min\left\{\beta + \frac{i}{2h} f(\OPT), F(x_B) \right\}                                                           \\
  &= \frac{1}{h} \sum_{i=1}^{\lfloor \gamma \rfloor}\left(\beta + \frac{i}{2h}f(\OPT)\right)
      + \frac{1}{h}\left(h - \lfloor \gamma \rfloor \right)F(x_B)                                                                                     \\
  &= \frac{1}{h} \left[ \lfloor \gamma \rfloor \left(\beta + \frac{1+\lfloor\gamma\rfloor}{4h} f(\OPT)\right) + (h-\lfloor \gamma \rfloor) F(x_B) \right] \\
  &\leq \frac{1}{h} \left[  \gamma  \left(\beta + \frac{1+\gamma}{4h} f(\OPT)\right) + (h- \gamma ) F(x_B) \right]                                        \\
  &= F(x_B) + \frac{1}{h} \frac{2h (F(x_B)-\beta)}{f(\OPT)} \left[ \frac{1+\frac{2h(F(x_B)-\beta)}{f(\OPT)}}{4h}f(\OPT) - (F(x_B) - \beta) \right]  \\
  &= F(x_B) - \frac{1}{f(\OPT)} (F(x_B)-\beta)^2 + \frac{1}{2h}(F(x_B)-\beta)\enspace,
\end{aligned}
\end{equation}
where the inequality follows from the fact that the function $g(z)\coloneqq z (\beta + \frac{1+z}{4h}f(\OPT)) + (h - z)F(x_B)$ is increasing for $z\in [\lfloor \gamma \rfloor,\gamma]$ because
\begin{align*}
\frac{d}{dz}g(z) &= \beta + \frac{1+2z}{4h}f(\OPT) - F(x_B)     \\
                 &\geq \beta + \frac{2\gamma}{4h}f(\OPT) - F(x_B) \\
                 &= 0\enspace.
\end{align*}
%
Combining \cref{eq:upperBoundAverageFxBi} with \cref{lem:averageXBIsCloseToXB}, we get
%
\begin{equation}\label{eq:fxBBetaDeltaIneq}
\frac{1}{f(\OPT)} (F(x_B) - \beta)^2 - \frac{1}{2h}(F(x_B)-\beta) - 4\Delta f(\OPT) \leq 0\enspace.
\end{equation}

By the definition of $\beta$ we have $\beta \geq F(x_B)- \frac{1}{2}f(\OPT)$, and hence $F(x_B)-\beta \leq \frac{1}{2}f(\OPT)$. We use this to bound the middle term of the above inequality, which leads to
\begin{equation}\label{eq:fxBBetaDeltaIneqRed}
\frac{1}{f(\OPT)} (F(x_B) - \beta)^2 - \left(\frac{1}{4h} + 4\Delta\right) f(\OPT) \leq 0\enspace.
\end{equation}

To obtain a lower bound on $\Delta$, we now derive an upper bound on $\beta$, which we will then use, together with the lower bound on $F(x_B)$ provided by \cref{lem:xBLowerBound}, to eliminate both $\beta$ and $F(x_B)$ in \cref{eq:fxBBetaDeltaIneqRed}.

To upper bound $\beta$, we observe that
\begin{align*}
\left( \frac{1}{2} + \Delta \right) f(\OPT)
  &= f(R)                                                                                                      \\
  &\geq F\left(x_B^{i^*} + \left(1-\frac{i^*}{h}\right)\characteristic_{\OPT_B}\right)                                    \\
  &\geq F(x_B^{i^*}) + \left(1 - \frac{i^*}{h}\right)\left(F\left(x_B\vee \characteristic_{\OPT_B}\right) - F(x_B)\right) \\
  &\geq F(x_B^{i^*}) + \left(1 - \frac{i^*}{h}\right)\left(\frac{1}{2} - \Delta\right)f(\OPT)                  \\
  &= \beta + \left( \frac{1}{2} - \Delta + \frac{i^*}{h}\Delta\right) f(\OPT)                                  \\
  &\geq \beta + \left(\frac{1}{2} - \Delta \right) f(\OPT) \enspace,                              \\
\end{align*}
where the used inequalities and equalities hold due to the following. The first inequality follows from the fact that the point $y\coloneqq x_B^i + (1-\frac{i^*}{h})\characteristic_{\OPT_B}$ satisfies $y\in P_M$, and \cref{lem:losslessRounding} then implies that there is an independent set $I\subseteq \supp(y)$ with $f(I) \geq F(y)$; finally, because $\supp(y)\subseteq Q\cup \cN_B$, this implies that $I$ is a candidate set for Bob to return.
The second inequality is a consequence of \cref{item:FVeeWedgeDimReturns} of \cref{lem:FSubmodularity} and $f(\varnothing)\geq 0$.
The third follows by \cref{item:xBWithOptB} of \cref{lem:boundNonMixedSols}.
The second equality is due to the definition of $\beta$.
The last inequality drops the non-negative term $\frac{i^*}{h}\Delta f(\OPT)$.
By reordering the terms on the leftmost side and rightmost side of the above relation, we obtain
\begin{equation*}
\beta \leq 2\Delta f(\OPT)\enspace.
\end{equation*}

Using this upper bound on $\beta$ and the lower bound on $F(x_B)$ given by \cref{lem:xBLowerBound} within \cref{eq:fxBBetaDeltaIneqRed}, and dividing by $f(\OPT)$, we obtain
\begin{equation*}
\left( \frac{1}{6} - \frac{11}{3} \Delta\right)^2 - \left( \frac{1}{4h} + 4\Delta\right) \leq 0\enspace.
\end{equation*}
For $h\geq 125$ this implies $\Delta\geq 0.005$, as desired.
\end{proof}


